Forces and pressures in adsorbing partially directed walks

Polymers in confined spaces lose conformational entropy. This induces a net repulsive entropic force on the walls of the confining space. A model for this phenomenon is a lattice walk between confining walls, and in this paper a model of an adsorbing partially directed walk is used. The walk is placed in a half square lattice $L^2_+$ with boundary $\partial L^2_+$, and confined between two vertical parallel walls, which are vertical lines in the lattice, a distance $w$ apart. The free energy of the walk is determined, as a function of $w$, for walks with endpoints in the confining walls and adsorbing in $\partial L^2_+$. This gives the entropic force on the confining walls as a function of $w$. It is shown that there are zero force points in this model and the locations of these points are determined, in some cases exactly, and in other cases asymptotically.

==> Fig3.tex <==
\beginpicture

\setcoordinatesystem units <1.5pt,1.5pt> point at 0 0

\setplotarea x from -80 to 150, y from -10 to 100
\setplotarea x from -10 to 150, y from -10 to 100

\color{Tan}
\setplotsymbol ({$\cdot$})

\grid 16 11


\color{black}
\setplotsymbol ({\large$\cdot$})
\plot 0 -10 0 100 /
\plot 0 0 150 0 /


\color{RoyalBlue}
\setplotsymbol ({\small$\bullet$})
\plot 0 0 0 10 0 20 10 20 10 10 10 0 10 0 20 0 30 0 30 10 30 20 30 30 30 40 30 50 30 60 30 70 30 80
40 80 40 70 50 70 50 60 50 50 60 50 60 40 60 30 70 30 70 40 80 40 80 50 90 50 90 40 90 30 90 20
90 10 90 0 100 0 100 10 100 20 110 20 120 20 120 30 120 40 130 40 130 50 140 50     /

\color{blue}
\multiput {\LARGE$\bullet$} at 
0 0 0 10 0 20 10 20 10 10 10 0 10 0 20 0 30 0 30 10 30 20 30 30 30 40 30 50 30 60 30 70 30 80
40 80 40 70 50 70 50 60 50 50 60 50 60 40 60 30 70 30 70 40 80 40 80 50 90 50 90 40 90 30 90 20
90 10 90 0 100 0 100 10 100 20 110 20 120 20 120 30 120 40 130 40 130 50 140 50     /


\color{black}
\setplotsymbol ({\small$\cdot$})
\arrow <10pt> [.2,.67] from 140 0 to 140 48
\arrow <10pt> [.2,.67] from 0 90 to 140 90

\put {\Large$h$} at 135 25
\put {\Large$w$} at 75 95
\multiput {\Large$a$} at 15 -5 25 -5 95 -5 /

\color{Sepia}
\multiput {\huge$\bullet$} at 0 0  140 50  /

\color{black}
\normalcolor

\endpicture


==> Fig4.tex <==
\beginpicture

\setcoordinatesystem units <1.5pt,1.5pt> point at 0 0

\setplotarea x from -80 to 150, y from -10 to 100
\setplotarea x from -10 to 150, y from -10 to 100

\color{Tan}
\setplotsymbol ({$\cdot$})

\grid 16 11


\color{black}
\setplotsymbol ({\large$\cdot$})
\plot 0 -10 0 100 /
\plot 0 0 150 0 /


\color{RoyalBlue}
\setplotsymbol ({\small$\bullet$})
\plot 0 0 0 10 0 20 10 20 10 10 10 0 10 0 20 0 30 0 30 10 30 20 30 30 30 40 30 50 30 60 30 70 30 80
40 80 40 70 50 70 50 60 50 50 60 50 60 40 60 30 70 30 70 40 80 40 80 50 90 50 90 40 90 30 90 20
90 10 90 0 100 0 100 10 100 20 110 20 120 20 120 30 120 40 130 40 130 50 140 50  140 40
140 30 140 20 140 10 140 0   /

\color{blue}
\multiput {\LARGE$\bullet$} at 
0 0 0 10 0 20 10 20 10 10 10 0 10 0 20 0 30 0 30 10 30 20 30 30 30 40 30 50 30 60 30 70 30 80
40 80 40 70 50 70 50 60 50 50 60 50 60 40 60 30 70 30 70 40 80 40 80 50 90 50 90 40 90 30 90 20
90 10 90 0 100 0 100 10 100 20 110 20 120 20 120 30 120 40 130 40 130 50 140 50   140 40
140 30 140 20 140 10 140 0   /


\color{black}
%\setplotsymbol ({\small$\cdot$})
%\arrow <10pt> [.2,.67] from 140 0 to 140 48
%\arrow <10pt> [.2,.67] from 0 90 to 140 90
%
%\put {\Large V} at 70 -6
%\put {\LARGE$w$} at 75 95
\multiput {\Large$a$} at 15 -5 25 -5 95 -5 /

\color{Sepia}
\multiput {\huge$\bullet$} at 0 0  140 0  /
%\multiput {\Huge$\bullet$} at 70 0  /

\color{black}
\normalcolor

\endpicture

